ParLS-PBO: A Parallel Local Search Solver for Pseudo Boolean Optimization

As a broadly applied technique in numerous optimization problems, recently, local search has been employed to solve Pseudo-Boolean Optimization (PBO) problem. A representative local search solver for PBO is LSPBO. In this paper, firstly, we improve LSPBO by a dynamic scoring mechanism, which dynamically strikes a balance between score on hard constraints and score on the objective function. Moreover, on top of this improved LSPBO , we develop the first parallel local search PBO solver. The main idea is to share good solutions among different threads to guide the search, by maintaining a pool of feasible solutions. For evaluating solutions when updating the pool, we propose a function that considers both the solution quality and the diversity of the pool. Furthermore, we calculate the polarity density in the pool to enhance the scoring function of local search. Our empirical experiments show clear benefits of the proposed parallel approach, making it competitive with the parallel version of the famous commercial solver Gurobi.

==> 4_Increasing_Diversity.tex <==
\section{More diversity}

\subsection{Configuration}

\subsection{Literal Assume}
We find that many instances of MIPLIB and PB16 have strong structures. We propose literal assume based unit propagation to simplify the PBO formula and diversify the worker, which can not only reduce the number of variables and constraints but also diversify the search direction, which is beneficial to find better solutions.

For the $2i-1$ and $2i$ th worker (i=1, ..., $\frac{nWorkers}{2}$ ), we fix the $LA_i$ of its PBO formula to 0 and 1, respectively, where $nWorkers$ is the number of workers and $LA_i$ is a randomly selected variable.
For each PBO formula with literal assume, we perform unit propagation on it, and our unit propagation rules are as follows:

step 1: Create a queue $q$ to which we add the fixed variable $LA_i$ and its corresponding assignment $v_i$ ,which is resulted from literal assume.

step 2: Take the fixed variable $x_k$ and its corresponding assignment $v_k$ from $q$, check for each constraint in which $x_k$ occurs, and reduce the constraint based on $v_i$. 
Specifically, assume that the constraint is $\sum_{i=0}^n a_i\cdot l_i \geq k_j$ and let $S$ denotes $\sum_{i=0}^n a_i$. Let $a_i=0$; If $l_i=x_i$ and $v_i=1$, or if $l_i= \neg x_i$ and $v_i=0$, then $k_j= k_j - a_i$. If $k_j \leq 0$, then the constraint can be deleted; if $S-a_{k'}+ 1 \leq k_j$, then $l_{k'}$ can be deduced to be 1, and $x_{k'}$ and the corresponding value will be added to the variable queue.

step 3: Repeat step 2 until the queue is empty.

% \begin{table}[h]
%     \begin{tabular}{l|llll} \hline
%     \textbf{benchmark} & \#inst & up\_var    & up\_con & up\_time \\ \hline
%     MWCB               & 24     & 0.9999964 & 0.9999907 & 14.91    \\
%     WSNO               & 18     & 0.9999997 & 0.9999941          & 3.0      \\
%     SAP                & 21     & 0.9967233 & 0.9926792 & 0.03     \\
%     MIPLIB             & 252    & 0.923465 & 0.9308294 & 0.43    \\
%     PB16               & 1524   & 0.8776243 & 0.8812923 & 0.05     \\ \hline
%     \textbf{All}       & 1839   & 0.8881987 & 0.8922057  & 0.29     \\ \hline
%     \end{tabular}
% \end{table}


==> Tables/5_2_sequential_sota.tex <==
% \begin{table*}[!ht]
% \centering
% % \small
% \begin{threeparttable}
% \caption{\label{tab:5_1_lspbo_lspboDcc}Comparison results between LS-PBO and LS-PBO-dynamic.}
% \label{tab:sequential}
% \begin{tabular}{c|c|cccc|cccc}
% \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{Benchmark}} & \multicolumn{1}{c|}{\multirow{3}{*}{\#ins}} & \multicolumn{4}{c|}{300s}   & \multicolumn{4}{c}{3600s}  \\ \cline{3-10} 

% \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{2}{c}{LS-PBO} & \multicolumn{2}{c|}{LS-PBO-dynamic} & \multicolumn{2}{c}{LS-PBO} & \multicolumn{2}{c}{LS-PBO-dynamic} \\ \cline{3-4}\cline{5-6}\cline{7-8}\cline{9-10}

% \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{Win} & \multicolumn{1}{c}{Score} & \multicolumn{1}{c}{Win} & \multicolumn{1}{c|}{Score}  & \multicolumn{1}{c}{Win} & \multicolumn{1}{c}{Score} & \multicolumn{1}{c}{Win} & \multicolumn{1}{c}{Score} \\ \hline
% Real-World    & 63      & 28    & 0.9787  & \textbf{41}      & \textbf{0.9878}   & \textbf{42}       & \textbf{0.9916}  & 37                  & 0.9911          \\
% MIPLIB        & 252     & 114   & 0.7845  & \textbf{184}     & \textbf{0.8357}   & 117               & 0.8158           & \textbf{198}        & \textbf{0.8691} \\
% PB16          & 1524    & 757   & 0.7035  & \textbf{1048}    & \textbf{0.737}    & 894               & 0.7671           & \textbf{1106}       & \textbf{0.7873} \\ 
% \hline
% Total         & 1839    & 899   & 0.724   & \textbf{1273}    & \textbf{0.7591}   & 1053              & 0.7814           & \textbf{1341}       & \textbf{0.8055}  \\ \hline

% \end{tabular}
% \end{threeparttable}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{\label{tab:5_1_lspbo_lspboD}
% Performance evaluation between~\lspbodym{} and sequential SOTA academic solvers.}
% % Comparison results between \lspbodym{} and academic solvers.}

% \setlength\tabcolsep{2.5pt}
% \renewcommand\arraystretch{1.1}
% \begin{tabular}{cccccccccccccc}
% \hline
% \multirow{2}{*}{Benchmark} & \multirow{2}{*}{\#Ins} & \multicolumn{2}{c}{\lspbo} & \multicolumn{2}{c}{\lspbodeci} & \multicolumn{2}{c}{\scip} & \multicolumn{2}{c}{\hybrid} & \multicolumn{2}{c}{\pboihs} & \multicolumn{2}{c}{\lspbodym}\\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}
% & & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$}
% & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$}\\
% \hline
% \multicolumn{14}{c}{cutoff=300s}\\
% \hline
% Real-World & 63 & 24 & 0.976 & 11 & 0.5465 & 0 & 0.1264 & 3 & 0.1095 & 2 & 0.2773 & \textbf{48} & \textbf{0.9956} \\
% MIPLIB & 252 & 84 & 0.7584 & 86 & 0.7364 & 104 & 0.6182 & 61 & 0.578 & 95 & 0.7575 & \textbf{138} & \textbf{0.8145} \\
% PB16 & 1524 & 626 & 0.6775 & 655 & 0.6849 & 847 & 0.6938 & 693 & 0.6311 & 912 & \textbf{0.8084} & \textbf{948} & 0.7507 \\
% Total & 1839 & 734 & 0.6988 & 752 & 0.6872 & 951 & 0.664 & 757 & 0.6059 & 1009 & \textbf{0.7832} & \textbf{1134} & 0.7679 \\
% \hline
% \multicolumn{14}{c}{cutoff=3600s} \\
% \hline
% Real-World & 63 & \textbf{39} & 0.99133 & 15 & 0.76759 & 0 & 0.1721 & 11 & 0.50283 & 5 & 0.40945 & \textbf{39} & \textbf{0.99148} \\
% MIPLIB & 252 & 86 & 0.79478 & 87 & 0.78305 & 134 & 0.67939 & 70 & 0.70531 & 111 & 0.79723 & \textbf{129} & \textbf{0.83772} \\
% PB16 & 1524 & 745 & 0.7394 & 745 & 0.74218 & 950 & 0.73906 & 779 & 0.72241 & 954 & \textbf{0.81734} & \textbf{1019} & 0.7974 \\
% Total & 1839 & 870 & 0.75562 & 847 & 0.74865 & 1084 & 0.71146 & 860 & 0.71255 & 1070 & 0.80061 & \textbf{1187} & \textbf{0.80958} \\
% \hline
% \end{tabular}
% \end{table*}



% \begin{table*}[t]
% \small
% \centering
% \caption{\label{tab:5_1_lspbo_lspboD}
% Performance evaluation between~\lspbodym{} and sequential SOTA solvers (The results of \lspbodeci{} are not presented due to the space limit. In fact, \lspbodeci{} is dominated by \nupbo{} and \lspbodym{}).}
% \setlength\tabcolsep{2.5pt}
% \renewcommand\arraystretch{1.1}
% \begin{tabular}{cccccccccccccccc}
% \hline
% \multirow{2}{*}{Benchmark} & \multirow{2}{*}{\#Ins} & \multicolumn{2}{c}{\scip} & \multicolumn{2}{c}{\hybrid} & \multicolumn{2}{c}{\pboihs} & \multicolumn{2}{c}{\nupbo} & \multicolumn{2}{c}{\gurobi(Comp.)} & \multicolumn{2}{c}{\gurobi(Heur.)} & \multicolumn{2}{c}{\lspbodym}\\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}
% & & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$}
% & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} & \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$}& \multicolumn{1}{c}{$\#win$} & \multicolumn{1}{c}{$avg_{sc^*}$} \\
% \hline
% \multicolumn{16}{c}{cutoff=300s}\\
% \hline
% Real-World & 63 & 0 & 0.126 & 3 & 0.109 & 2 & 0.266 & \textbf{46} & \textbf{0.972} & 4 & 0.289 & 4 & 0.292 & 29 & 0.977 \\
% MIPLIB & 252 & 88 & 0.614 & 53 & 0.572 & 81 & 0.741 & 116 & 0.844 & 152 & 0.838 & \textbf{165} &\textbf{0.849} & 101 & 0.803 \\
% PB16 & 1524 & 810 & 0.687 & 663 & 0.624 & 882 & 0.804 & 980 & 0.813 & 1071 & 0.84 & \textbf{1072} & \textbf{0.84} & 842 & 0.741 \\
% \hline
% \multicolumn{16}{c}{cutoff=3600s} \\
% \hline
% Real-World & 63 & 0 & 0.171 & 11 & 0.494 & 5 & 0.401 & \textbf{43} & \textbf{0.997} & 11 & 0.34 & 9 & 0.38 & 27 & 0.974 \\
% MIPLIB & 252 & 113 & 0.675 & 65 & 0.697 & 96 & 0.789 & 113 & 0.859 & 171 & 0.893 & \textbf{181} & \textbf{0.895} & 106 & 0.831 \\
% PB16 & 1524 & 906 & 0.734 & 729 & 0.715 & 939 & 0.814 & 1012 & 0.822 & 1138 & 0.86 & \textbf{1144} & \textbf{0.862} & 940 & 0.797 \\
% \hline
% \end{tabular}
% \end{table*}


\begin{table}[!h]
\small
\centering
\caption{\label{tab:5_1_lspbo_lspboD}
Performance evaluation between~\lspbodym{} and sequential SOTA solvers (The results of \lspbodeci{} are not presented due to the space limit. In fact, \lspbodeci{} is dominated by \nupbo{} and \lspbodym{}).}
\setlength\tabcolsep{2pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{cc|c|c|c|c|c|c|c}
\hline
\multirow{3}{*}{Benchmark} &\multirow{3}{*}{\#Ins} &\scip{} &\hybrid{} &\pboihs{} &\nupbo{} &\gurobi{}(Comp.) &\gurobi{}(Heur.) &\lspbodym{} \\
\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-9}
& &$\#win$ &$\#win$ &$\#win$ &$\#win$ &$\#win$ &$\#win$ &$\#win$ \\
& &$avg_{sc^*}$ &$avg_{sc^*}$ &$avg_{sc^*}$ &$avg_{sc^*}$ &$avg_{sc^*}$ &$avg_{sc^*}$ &$avg_{sc^*}$ \\
\hline
\multicolumn{9}{c}{cutoff=300s}\\
\hline 
\multirow{2}{*}{Real-World} &\multirow{2}{*}{63} & 0 & 3 & 2 & \textbf{46} & 4 & 4 & 29 \\
 & & 0.126  & 0.109  & 0.266  & \textbf{0.972}  & 0.289  & 0.292  & 0.977 \\
\hline
\multirow{2}{*}{MIPLIB} &\multirow{2}{*}{252}& 88 & 53& 81& 116& 152& \textbf{165}& 101\\
 &   & 0.614  & 0.572  & 0.741  & 0.854  & 0.838  &\textbf{ 0.849}  & 0.803 \\
\hline
\multirow{2}{*}{PB16} &\multirow{2}{*}{1524} & 810 & 663 & 882& 980  & 1071 & \textbf{1072} & 842\\
&   & 0.687  & 0.624  & 0.804  & 0.813 & 0.84  & \textbf{0.84}  & 0.741 \\
\hline
\multicolumn{9}{c}{cutoff=3600s} \\
\hline
\multirow{2}{*}{Real-World} &\multirow{2}{*}{63}& 0& 11 & 5& \textbf{43}& 11& 9& 27\\
 &   & 0.171 & 0.494  & 0.401  & \textbf{0.997}  & 0.34  & 0.38  & 0.974 \\
 \hline
\multirow{2}{*}{MIPLIB} &\multirow{2}{*}{252}& 113& 65& 96& 113& 171 & \textbf{181}& 106\\
&   & 0.675  & 0.697  & 0.789  & 0.859  & 0.893 & \textbf{0.895}  & 0.831 \\
\hline
\multirow{2}{*}{PB16} &\multirow{2}{*}{1524}& 906& 729& 939& 1012& 1138& \textbf{1144}& 940\\
&   & 0.734  & 0.715  & 0.814  & 0.822  & 0.86  & \textbf{0.862}  & 0.797 \\
\hline
\end{tabular}
\end{table}
